Cut-elimination for the mu-calculus with one variable

We establish syntactic cut-elimination for the one-variable fragment of the modal mu-calculus. Our method is based on a recent cut-elimination technique by Mints that makes use of Buchholz' Omega-rule.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{D. Miller and Z. \'Esik (Eds.):  Fixed Points\\
in Computer Science 2012 (FICS 2012)\\
EPTCS 77, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.77.7}{10.4204/EPTCS.77.7}}

